Grounding Characters and Places in Narrative Texts

Tracking characters and locations throughout a story can help improve the understanding of its plot structure. Prior research has analyzed characters and locations from text independently without grounding characters to their locations in narrative time. Here, we address this gap by proposing a new spatial relationship categorization task. The objective of the task is to assign a spatial relationship category for every character and location co-mention within a window of text, taking into consideration linguistic context, narrative tense, and temporal scope. To this end, we annotate spatial relationships in approximately 2500 book excerpts and train a model using contextual embeddings as features to predict these relationships. When applied to a set of books, this model allows us to test several hypotheses on mobility and domestic space, revealing that protagonists are more mobile than non-central characters and that women as characters tend to occupy more interior space than men. Overall, our work is the first step towards joint modeling and analysis of characters and places in narrative text.

==> acl/002data.tex <==
\section{Data}
\label{sec:data}
Our primary source of data is a sample  of English-language books from Project Gutenberg. These titles span multiple centuries, index different genres, and contain a mix of fiction and narrative non-fiction.  All works are in the public domain in the United States and are able to be openly published along with our annotations.


%The full text of books from Project Gutenberg is of high quality, a key factor in steering our choice towards this data source. Moreover, the collection is diverse: titles span multiple centuries, index different genres, are a mix of fiction and non-fiction, and written by authors of a diverse demographic. A summary of descriptive statistics of books in Project Gutenberg is given in~\autoref{tab:descriptive}.

%\input{acl/tables/tab-descriptive.tex}


%Our book collection is then processed with the bookNLP pipeline to additionally mark up the text with entities, their types, their coreferences, and their inferred gender. For the definitions of entities and entity types that bookNLP identifies, please refer to the paper. Text spans marked up as "PER" entity by bookNLP are deemed as candidate characters in the story; on the other hand, spans marked up as one of "LOC", "FAC", or "GPE" are deemed as candidate places in the story. We then find all instances in the collection where a candidate character is collocated with the candidate place name within 10 tokens of each other. These instances form the basis for the task described next.

==> acl/old_task_descriptions.tex <==
After filtering out the examples in Task a (described in~\autoref{sec:filtering-task}), this task seeks to categorize the relationship between the character and the place. In total there are $9$ categories whose definitions are given in~\autoref{tab:spatial-task-definitions}. We formalized these categories to be sufficiently expressive about the different scenarios after initial rounds of grounded coding on small samples taken from books.

\begin{comment}
\paragraph{IN.} 
When the character $C$ is at the place $L$ (e.g., \word{at \place{the restaurant}}), in the place (e.g., \word{in \place{the building}}), or on the place (e.g., \word{on \place{the front porch}}).  Lexical cues of the character's position are not always explicit and need to be inferred such as in the following example.

\begin{itemize}
    \item[] From the windows of \place{the room where I slept} \character{I} had a view of one of these old places  
\end{itemize}

In this case, the character could only describe the view from inside the room and hence is \enttype{IN} the room.
\end{comment}
\paragraph{IN.} This category is a direct judgment of whether a character is grounded at a known place in the story. Lexical cues about a character's position are not always explicit and need to be inferred such as in the following example.

\begin{quote}{George Borrow, Lavengro}
From the windows of \place{the room where I slept} \character{I} had a view of one of these old places 
\end{quote}

\paragraph{NEAR.} This label is highly contextual and relative: large absolute distance between a character and a place can be deemed near depending on the contextual description. To illustrate this category with an example, consider the following:

\begin{quote}{Jules Verne, In search of the castaways}
But \place{the swollen waters of the river} bar our progress . \character{I} would pay its weight in gold for a raft that would transport us to the other side! 
\end{quote}

Before starting their journey, the character is near the river.

\paragraph{THRU.} Unlike previous categories in which characters are assumed stationary, this category implies motion. Consider the following example:

\begin{quote}{Charlotte Brame, Dora Thorne}
    If you will not dance with me again , will you walk through \place{the rooms}? `` Many admiring glances followed \character{them} -- a handsomer pair was seldom seen .
\end{quote}

In this example, the couple (referenced as ``them'') is moving through the rooms.

\paragraph{TO(C).} This is another category which implies character in motion. A character moves towards a destination such as in the following example. 
\begin{quote}{Molly Seawell, Francezka}
    Within a month from the time of Gaston Cheverny 's return from Brabant \character{he} was sent to \place{Poland} and East Prussia on an errand that might last a month and might last a year. He went gallantly enough. 
\end{quote}

The last sentence makes it clear that the character (referred by ``he") moves towards and Poland.

\paragraph{TO(U).} The difference between this and the previous category is that the character is unlikely to reach the destination. To illustrate with an example, consider the following.

\begin{quote}{Alice Emerson, Betty Gordon at Bramble Farm}
    She was to take \character{Betty} \place{upstairs} and let her make herself neat for supper
\end{quote}

It's unclear in the limited context given, if the character (Betty) went to the place (upstairs).

\paragraph{FROM} To capture the situation when the character left a place or came from a place, we introduce this category. Consider the following example,

\begin{quote}{Alfred Church, Lords of the world}
`` we came across the eparch's wagon as it was on its way to Larissa from \place{the coast}''. As there was clearly more wine than \character{he} could use -- it is the one fault of Lesbian wine that it does not keep very well.
\end{quote}

\paragraph{NO REL.} Besides the definition in~\autoref{tab:spatial-task-definitions}, this category is assigned if there is no sufficient information to deduce the relationship between $C$ and $L$. For example,

\begin{quote}{Jane Porter, The scottish chiefs}
The earl inquired anxiously for Sir William Wallace, and asked if he might expect him soon at \place{Bothwell}. "\character{He} can not yet come, my lord," replied Halbert. 
\end{quote}

The spatial relationship between the character (he) and the location (Bothwell) has not been asserted yet and hence the label should be \enttype{NO REL}. Hypothetical spatial relationships (\character{Peter} will travel to \place{London}) describe a speculative link between the two entities in questions and therefore are also given the label of \enttype{NO REL}.

\paragraph{NEG.} This category is semantically opposite to \enttype{IN}. To explain further, consider the following example.

\begin{quote}{James Driscoll, The Brighton boys in the Argonne forest}
There being no sign of \character{the spy} on \place{the ridge top}, the searchers spread out and two of them came
\end{quote}

At narrative time, the candidate character (the spy) is not present at the candidate location (the ridge top) marked. 

\paragraph{UNCERTAIN.}  To capture the situation where uncertainty in the grounding of the character is implied in the text. For example,

\begin{quote}{Lester Chadwick, Baseball Joe in the Big League}
    ``Was \character{he} in there?'' asked Joe, nodding toward \place{the billiard room}, where he had met several of the players. ``No. I don't know where he is,'' went on the manager.
\end{quote}

Here, the manager describes with uncertainty the whereabouts of the character (he).

The next two subtasks consider the time for which the spatial relationship exists(\autoref{sec:temporal-span-classification-task}) and the current status of the relationship with respect to the narrative time(\autoref{sec:narrative-tense-classification-task}).


==> acl/tables/tab-annotation-errors.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|l}
        \toprule
        Disagreement reason & \# examples \\
        \midrule
        Definition misunderstanding & 20 \\
        Genuine ambiguity & 15 \\
        Specific Vs Generic & 6 \\
        Label ambiguity & 5 \\
        Other & 4\\
        \bottomrule
    \end{tabular}
    \caption{Distribution of the sources of disagreement in annotation}
    \label{tab:annotation-errors}
\end{table}

==> acl/tables/tab-annotations.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|r}
        \toprule
        Category & Count \\
        \midrule
        IN & 389 \\
        NEAR & 91 \\
        THRU & 30 \\
        TO(C) & 54 \\
        To(U) & 25 \\
        FROM & 40 \\
        NO REL & 319 \\
        NEG & 18 \\
        UNCERTAIN & 6 \\
        \bottomrule
    \end{tabular}
    \caption{Distribution of labels in the annotated set. A further 295 examples were filtered out as invalid either because of errors in identifying characters and locations, or because of lack of specificity in marking up characters and locations.}
    \label{tab:annotation-distribution}
\end{table}

==> acl/tables/tab-descriptive.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|l}
        Statistic & Value \\
        \hline
        Number of documents & 19532 \\
        Max tokens in document & \\
        Min tokens in document & \\
        Total tokens in corpus & \\
    \end{tabular}
    \caption{Descriptive statistics for the Project Gutenberg corpus}
    \label{tab:descriptive}
\end{table}

==> acl/tables/tab-indoor-proclivity-time.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
        \toprule
        Year range & he/him/his & she/her\\
        \midrule
        1700-1800 & 0.56 & 0.68\\
        1800-1850 & 0.6 & 0.71\\
        1850-1900 & 0.56 & 0.66\\
        1900-1950 & 0.48 & 0.59\\
        \bottomrule
    \end{tabular}
    \caption{Proclivity of characters towards occupying indoor spaces over time. We find that characters are less inclined to reside in indoor spaces over time but female characters are as likely to be indoors when compared to male characters. }
    \label{tab:indoor-proclivity-time}
\end{table}
